A formal specification of the desired software behaviour of the Princess Marijke lock complex

The Princess Marijke lock complex is a large lock and water-protection installation in the Netherlands between the river Rhine and the Amsterdam-Rijnkanaal -- a large waterway connecting the Rhine to the port of Amsterdam. The lock complex consists of two independent locks and a moveable flood-protection barrier. Ensuring safe control of the lock complex is of utmost importance to guarantee both flood-protection and reliable ship operations. This paper gives a precise, formal description of the software control of the lock complex in less than 400 lines of mCRL2 code. This description can act as a blueprint on how the software of this lock complex needs to be constructed. Moreover, using model checking, 53 software requirements are shown to be valid, ensuring that the formal description of the behaviour is correct with regard to these properties and is unlikely to contain mistakes and oversights.

==> model/runreq <==
mcrl22lps marijkesluizen_wfaults_spec.mcrl2 scratch/temp$1.lps -v --timings &&
lpsfununfold scratch/temp$1.lps -v | lpssuminst | \
   lpsrewr -v | lpsconstelm -v | lpsparelm -v > scratch/temp2$1.lps &&
lps2pbes scratch/temp2$1.lps -frequirements/$1.mcf -v scratch/temp$1.pbes &&
pbesconstelm -v -c scratch/temp$1.pbes | pbesrewr | \
  pbesparelm -v > scratch/temp1$1.pbes &&
pbesrewr -pquantifier-inside scratch/temp1$1.pbes -v | \
  pbesrewr -pquantifier-one-point -v | pbesrewr | pbesrewr -pquantifier-all -v | \
  pbesrewr | pbesconstelm -cv | pbesrewr | pbesparelm -v | pbesconstelm -cve | \
  pbesrewr > scratch/$1.pbes &&
pbessolvesymbolic --memory-limit=$2 scratch/$1.pbes -v --split-conditions \
  --cached -rjittyc --groups=used --chaining --saturation --timings
echo -----------------------------------------------------------------------
echo Checked formula $1.mcf
echo -----------------------------------------------------------------------

